Structured $H_\infty$-Optimal Control for Nested Interconnections: A State-Space Solution

If imposing general structural constraints on controllers, it is unknown how to design $H_\infty$-controllers by convex optimization. Under a so-called quadratic invariance structure of the generalized plant, the Youla parametrization allows to translate the structured synthesis problem into an infinite-dimensional convex program. Nested interconnections that are characterized by a standard plant with a block-triangular structure fall into this class. Recently it has been shown how to design optimal $H_2$-controllers for such nested structures in the state-space by solving algebraic Riccati equations. In the present paper we provide a state-space solution of the corresponding output-feedback $H_\infty$ synthesis problem without any counterpart in the literature. We argue that a solution based on Riccati equations is - even for state-feedback problems - not feasible and we illustrate our results by means of a simple numerical example.

==> exa1a.tex <==
-0.01 0.26563 0.26277
-0.078621 0.72089 0.73467
-0.14724 0.99219 1.0044
-0.21586 1.1953 1.2156
-0.28448 1.0204e-06 1.3955
-0.3531 1.0227e-06 1.5549
-0.42172 1.0249e-06 1.6998
-0.49034 1.0269e-06 1.8336
-0.55897 1.0286e-06 1.9587
-0.62759 1.0304e-06 2.0766
-0.69621 1.032e-06 2.1886
-0.76483 2.2578 2.2954
-0.83345 2.3516 2.3979
-0.90207 2.4531 2.4965
-0.97069 2.5469 2.5918
-1.0393 2.6328 2.684
-1.1079 2.7266 2.7735
-1.1766 2.8047 2.8606
-1.2452 2.8906 2.9454
-1.3138 2.9766 3.0282
-1.3824 3.0547 3.1091
-1.451 3.1328 3.1883
-1.5197 3.2031 3.2659
-1.5883 3.2813 3.342
-1.6569 3.3516 3.4168
-1.7255 3.4219 3.4902
-1.7941 3.5 3.5625
-1.8628 3.5625 3.6336
-1.9314 3.6328 3.7036
-2 3.7031 3.7727


==> exa1b.tex <==
-0.01 84.017 8.5762 7.1365 6.3078
-0.078621 83.929 8.3567 6.8812 6.0121
-0.14724 83.842 8.1333 6.6144 5.6886
-0.21586 83.754 7.9055 6.3454 5.3294
-0.28448 83.666 7.6734 6.0381 4.8835
-0.3531 83.579 7.4368 5.7273 4.487
-0.42172 83.492 7.1962 5.4439 4.029
-0.49034 83.405 6.9522 5.1008 3.5873
-0.55897 83.318 6.7061 4.7588 3.1906
-0.62759 83.232 6.4597 4.4298 2.8563
-0.69621 83.145 6.2153 4.1243 2.6083
-0.76483 83.059 5.9757 3.8504 2.5745
-0.83345 82.973 5.7436 3.6135 2.6159
-0.90207 82.887 5.522 3.417 2.6832
-0.97069 82.802 5.3133 3.2642 2.7625
-1.0393 82.716 5.1194 3.1705 2.8477
-1.1079 82.631 4.9422 3.1677 2.9357
-1.1766 82.546 4.7828 3.1835 2.9989
-1.2452 82.462 4.6423 3.2501 3.0936
-1.3138 82.376 4.5215 3.3218 3.1845
-1.3824 82.292 4.421 3.3967 3.2702
-1.451 82.208 4.3415 3.4733 3.3508
-1.5197 82.124 4.2834 3.5498 3.428
-1.5883 82.04 4.247 3.6257 3.5023
-1.6569 81.956 4.232 3.7001 3.5739
-1.7255 81.872 4.1951 3.7741 3.6434
-1.7941 81.789 4.2293 3.8469 3.7111
-1.8628 81.706 4.2676 3.9183 3.7772
-1.9314 81.623 4.3107 3.9883 3.8419
-2 81.54 4.3578 4.0569 3.9054


==> exa2a.tex <==
-0.01 0.26563 1.0367
-0.078621 0.72089 2.7936
-0.14724 0.99219 3.7651
-0.21586 1.1953 4.5205
-0.28448 1.0204e-06 5.1645
-0.3531 1.0227e-06 5.7388
-0.42172 1.0249e-06 6.2649
-0.49034 1.0269e-06 6.7555
-0.55897 1.0286e-06 7.2188
-0.62759 1.0304e-06 7.6605
-0.69621 1.032e-06 8.0846
-0.76483 2.2578 8.494
-0.83345 2.3516 8.8911
-0.90207 2.4531 9.2777
-0.97069 2.5469 9.6552
-1.0393 2.6328 10.025
-1.1079 2.7266 10.387
-1.1766 2.8047 10.743
-1.2452 2.8906 11.094
-1.3138 2.9766 11.44
-1.3824 3.0547 11.781
-1.451 3.1328 12.118
-1.5197 3.2031 12.451
-1.5883 3.2813 12.781
-1.6569 3.3516 13.108
-1.7255 3.4219 13.432
-1.7941 3.5 13.753
-1.8628 3.5625 14.072
-1.9314 3.6328 14.388
-2 3.7031 14.703


==> exa2b.tex <==
-0.01 84.048 8.652 7.2248 6.406
-0.078621 84.171 8.9526 7.6319 6.7861
-0.14724 84.295 9.2488 7.8844 7.1495
-0.21586 84.418 9.4471 8.207 7.5001
-0.28448 84.542 9.7407 8.6017 7.8405
-0.3531 84.666 10.031 8.9123 8.1727
-0.42172 84.789 10.318 9.2181 8.498
-0.49034 84.913 10.603 9.5199 8.8176
-0.55897 85.037 10.885 9.8181 9.1323
-0.62759 85.161 11.165 10.021 9.4428
-0.69621 85.285 11.443 10.319 9.7497
-0.76483 85.409 11.719 10.614 9.9608
-0.83345 85.533 11.994 10.906 10.267
-0.90207 85.657 12.268 11.196 10.571
-0.97069 85.782 12.54 11.483 10.872
-1.0393 85.906 12.811 11.769 11.17
-1.1079 86.03 13.081 12.054 11.467
-1.1766 86.155 13.35 12.337 11.761
-1.2452 86.279 13.618 12.618 12.053
-1.3138 86.404 13.885 12.898 12.344
-1.3824 86.528 14.151 13.177 12.634
-1.451 86.653 14.417 13.455 12.922
-1.5197 86.777 14.682 13.732 13.208
-1.5883 86.902 14.947 14.009 13.494
-1.6569 87.027 15.21 14.284 13.778
-1.7255 87.151 15.474 14.559 14.062
-1.7941 87.276 15.736 14.832 14.345
-1.8628 87.401 15.999 15.105 14.626
-1.9314 87.526 16.26 15.378 14.907
-2 87.651 16.522 15.65 15.187

